Learning Groupwise Multivariate Scoring Functions Using Deep Neural Networks

While in a classification or a regression setting a label or a value is assigned to each individual document, in a ranking setting we determine the relevance ordering of the entire input document list. This difference leads to the notion of relative relevance between documents in ranking. The majority of the existing learning-to-rank algorithms model such relativity at the loss level using pairwise or listwise loss functions. However, they are restricted to univariate scoring functions, i.e., the relevance score of a document is computed based on the document itself, regardless of other documents in the list. To overcome this limitation, we propose a new framework for multivariate scoring functions, in which the relevance score of a document is determined jointly by multiple documents in the list. We refer to this framework as GSFs -- groupwise scoring functions. We learn GSFs with a deep neural network architecture, and demonstrate that several representative learning-to-rank algorithms can be modeled as special cases in our framework. We conduct evaluation using click logs from one of the largest commercial email search engines, as well as a public benchmark dataset. In both cases, GSFs lead to significant performance improvements, especially in the presence of sparse textual features.

==> ScoringLossDiagram.tex <==
  \begin{center}
    \begin{tikzpicture}[scale=0.85, every node/.style=transform shape,minimum height=18pt]
      %
      % Legend on the left
      %
      \node[align=center](InptLabel)
           { Inputs };
      \node[align=center](ScFnLabel)
           [above=17pt of InptLabel]
           { Scoring\\ function};
      \node[align=center](LossLabel)
           [above=17pt of ScFnLabel]
           { Loss };
      %
      % Stack for pointwise scoring / pointwise loss
      %
      \node[draw,dashed,align=center](InptPtPt1)
           [right=10pt of InptLabel]
           { $q, d_1, y_1$ };
      \node[draw,align=center](ScFnPtPt1)
           [above=20pt of InptPtPt1]
           { $f(q, d_1)$ };
      \draw[->,line width=0.8pt](InptPtPt1) edge (ScFnPtPt1);
      \node[draw,align=center](LossPtPt1)
           [above=20pt of ScFnPtPt1]
           { $l(q, d_1, y_1)$ };
      \draw[->,line width=0.8pt](ScFnPtPt1) edge (LossPtPt1);
      \node[draw,dashed,align=center](InptPtPtN)
           [right=20pt of InptPtPt1]
           { $q, d_n, y_n$ };
      \node[draw,align=center](ScFnPtPtN)
           [above=20pt of InptPtPtN]
           { $f(q, d_n)$ };
      \draw[->,line width=0.8pt](InptPtPtN) edge (ScFnPtPtN);
      \node[draw,align=center](LossPtPtN)
           [above=20pt of ScFnPtPtN]
           { $l(q, d_n, y_n)$ };
      \draw[->,line width=0.8pt](ScFnPtPtN) edge (LossPtPtN);
      \path (LossPtPt1) -- node[auto=false]{\ldots} (LossPtPtN);
      \path (ScFnPtPt1) -- node[auto=false]{\ldots} (ScFnPtPtN);
      \path (InptPtPt1) -- node[auto=false](MidPtPt){\ldots} (InptPtPtN);
      \node[align=left](GraphPtPt)
           [below=10pt of MidPtPt]
           { (a) Pointwise scoring \\ \hphantom{(a)} Pointwise loss };
      %
      % Stack for pairwise scoring / pairwise loss
      %
      \node[draw,dashed,align=center](InptPrPr1)
           [right=40pt of InptPtPtN]
           { $q, d_{ij}, y_{ij}$ };
      \node[draw,align=center](ScFnPrPr1)
           [above=20pt of InptPrPr1]
           { $f(q, d_{ij})$ };
      \draw[->,line width=0.8pt](InptPrPr1) edge (ScFnPrPr1);
      \node[draw,align=center](LossPrPr1)
           [above=20pt of ScFnPrPr1]
           { $l(q, d_{ij}, y_{ij})$ };
      \draw[->,line width=0.8pt](ScFnPrPr1) edge (LossPrPr1);
      \node[draw,dashed,align=center](InptPrPrN)
           [right=20pt of InptPrPr1]
           { $q, d_{km}, y_{km}$ };
      \node[draw,align=center](ScFnPrPrN)
           [above=20pt of InptPrPrN]
           { $f(q, d_{km})$ };
      \draw[->,line width=0.8pt](InptPrPrN) edge (ScFnPrPrN);
      \node[draw,align=center](LossPrPrN)
           [above=20pt of ScFnPrPrN]
           { $l(q, d_{km}, y_{km})$ };
      \draw[->,line width=0.8pt](ScFnPrPrN) edge (LossPrPrN);
      \path (LossPrPr1) -- node[auto=false]{\ldots} (LossPrPrN);
      \path (ScFnPrPr1) -- node[auto=false]{\ldots} (ScFnPrPrN);
      \path (InptPrPr1) -- node[auto=false](MidPrPr){\ldots} (InptPrPrN);
      \node[align=left](GraphPrPr)
           [below=10pt of MidPrPr]
           { (b) Pairwise scoring \\ \hphantom{(b)} Pairwise loss };
      %
      % Stack for pointwise scoring / listwise loss
      %
      \node[draw,dashed,align=center](InptPtLs1)
           [right=40pt of InptPrPrN]
           { $q, d_1, y_1$ };
      \node[draw,dashed,align=center](InptPtLsN)
           [right=20pt of InptPtLs1]
           { $q, d_n, y_n$ };
      \path (InptPtLs1) -- node[auto=false](MidPtLs){\ldots} (InptPtLsN);
      \node[draw,align=center](ScFnPtLs1)
           [above=20pt of InptPtLs1]
           { $f(q, d_1)$ };
      \node[draw,align=center](ScFnPtLsN)
           [above=20pt of InptPtLsN]
           { $f(q, d_n)$ };
      \path (ScFnPtLs1) -- node[auto=false](MiMiPtLs){\ldots} (ScFnPtLsN);
      \node[draw,align=center](LossPtLs)
           [above=20pt of MiMiPtLs]  
           { $l(q, D, Y)$ };
      \draw[->,line width=0.8pt](InptPtLs1) edge (ScFnPtLs1);
      \draw[->,line width=0.8pt](ScFnPtLs1) edge (LossPtLs);
      \draw[->,line width=0.8pt](InptPtLsN) edge (ScFnPtLsN);
      \draw[->,line width=0.8pt](ScFnPtLsN) edge (LossPtLs);
      \node[align=left](GraphPtLs)
           [below=10pt of MidPtLs]
           { (c) Pointwise scoring \\ \hphantom{(c)} Listwise loss };
      %
      % Stack for groupwise scoring / listwise loss
      %
      \node[draw,dashed,align=center](InptLsLs)
           [right=40pt of InptPtLsN]
           { $q, D, Y$ };
      \node[draw,align=center](ScFnLsLs)
           [above=20pt of InptLsLs]
           { $f(q, D)$ };
      \draw[->,line width=0.8pt](InptLsLs) edge (ScFnLsLs);
      \node[draw,align=center](LossLsLs)
           [above=20pt of ScFnLsLs]  
           { $l(q, D, Y)$ };
      \draw[->,line width=0.8pt](ScFnLsLs) edge (LossLsLs);
      \node[align=left](GraphPtLs)
           [below=10pt of InptLsLs]
           { (d) Groupwise scoring \\ \hphantom{(d)} Listwise loss };
    \end{tikzpicture}
  \end{center}
  \vspace{-5mm}


==> intro.tex <==
%!TEX root=paper.tex
\section{Introduction}\label{sec:intro}

%\begin{figure*}
%  %\centering\includegraphics[scale=0.6]{./figure/ScoringLossDiagram.pdf}
%  \include{ScoringLossDiagram}
%  \caption{Schematic of some common \{scoring, loss\} combinations in learning-to-rank models. $q$ denotes the query. $d_i \in D, y_i \in Y$ denote a document at $i$-th rank and its relevance label, respectively. $d_{ij}, y_{ij}$ denote a pair of documents and their pairwise preference, respectively.}
%  \label{fig:scoringloss}
%\end{figure*}
%
% Relativity for ranking
%Ranking is the foundation of many information retrieval (IR) problems, including \emph{ad hoc} document retrieval, question answering, recommender systems, and many others. 
Unlike the traditional classification or regression setting, the main goal of a ranking problem is not to assign a label or a value to each individual document, but to determine the relative relevance among a list of them. A ranked list of documents is usually presented to users and the relevance of the top ranked documents influences the utility of the entire list more heavily~\cite{Chapelle+al:2009}. An ideal ranked list should be ordered by document relevance.
%The order of the documents highly influences the utility of the list and it is desirable to put more relevant documents at the top of the ranked list. 
% Thus, the notion of \emph{relativity} is crucial in a ranking problem.

%Different from other tasks like classification, ranking does not require each object to have meaningful labels.
%It only concerns about preferences.
%For example, in web search, we need to know how much a user prefer a document comparing to others, but not necessarily how relevant the document is to the query topic. 
%Therefore, relativity is the core of ranking.

% Relativity in LTR
How to model document relevance has been extensively studied, most recently in the learning-to-rank setting~\cite{liu2009learning}. In this setting, a scoring function that maps document feature vectors to real-valued scores is learned from training data. Documents are then ranked according to the predictions of the scoring function.
% Broadly speaking, in this paradigm, each query-document pair is represented by a feature vector. These feature vectors are used as input to learn a model to predict their relevance scores. The final list is then produced by sorting the documents by their predicted scores with respect to the query. 
Since what matters most is the document order, the majority of the learning-to-rank algorithms learn the scoring function using pairwise or listwise loss functions to capture the relative relevance between documents~\cite{burges2005learning, quoc2007learning, cao2007learning, Jun+Hang:2007}.
Such a loss guides the learning of the scoring function to optimize preferences between documents or an IR metric such as NDCG~\cite{Joachims:2002, Taylor+al:2008, burges2010ranknet}. Though effective, most of them are still restricted to the paradigm of \emph{univariate scoring functions}: the relevance score of a document to a query is computed independently of other documents in the list. %, as shown in Figure~\ref{fig:scoringloss} (a) and (c). 

%Thus, relativity among documents is modeled \emph{indirectly} through loss functions in the existing methods and this can be less optimal for ranking problems\footnote{It is interesting to note the connection of pointwise scoring to Robertsons' probability ranking principle (PRP)~\cite{Robertson:1977}. PRP states that documents should be ranked by their probability of relevance to the query. While highly cited and influential, this principle was recognized to be problematic by Robertson himself: ``The PRP works document-by-document, whereas the results should be evaluated request-by-request''~\cite{Robertson:1977}.}.

%%Example why, in practice, the pointwise input assumption is problematic.
% First, this setting has limited power to model cross-document interactions. 
%%Rephrased the search scenario example.
%Consider a search scenario where a user is searching for a name of a musical artist. If all the results returned by the query (e.g., \emph{calvin harris}) are recent, the user may be interested in the latest news or tour information. If, on the other hand, most of the query results are older (e.g., \emph{frank sinatra}), it is more likely that the user wants to learn about artist discography or biography.
%%Consider an email search scenario where a user is searching for an order number of a past online purchase. If all search results are recent, the user may just want to check the shipping information. If, on the other hand, all the results are old, it is more likely that the user wants the order receipt instead.
%%A scoring function under the pointwise input principle cannot take advantages of such context information.
% 
%Second, prior research suggests that preference judgments by comparing a pair of documents are faster to obtain, and are more consistent than the absolute ratings~\cite{Bennett+al:2008,ye2013combining,koczkodaj1996statistically}, 
%%it is natural to expect that modeling relative relevance among documents may be easier than modeling absolute relevance. Thus, 
%Thus, it can be beneficial to directly compare documents based on their features in a learning algorithm, in addition to indirect comparison through loss functions.
%
%Third, user interaction with search results shows strong comparison patterns, and better predictive capability is achieved when user actions are modeled in a relative fashion (e.g., SkipAbove)~\cite{Joachims+al:2005, Borisov+al:2016, yilmaz2014relevance, craswell2008experimental, dupret2008user, Chapelle+al:2009}. These indicate that users compare the clicked document to its surrounding documents prior to a click. In the unbiased learning-to-rank setting where clicks are debiased and used as ground-truth labels~\cite{Wang+al:2016, Joachims:WSDM17, Wang+al:2018}, a ranking model that uses the direct comparison mechanism can be more effective as it mimics the user behavior more faithfully.

% Propose unified ranking framework and 
% Given these observations, 
Recently, pairwise scoring functions, which take two documents as input and output a probability of preference for the two input documents 
% as shown in Figure~\ref{fig:scoringloss} (b), 
were introduced in~\cite{Dehghani:SIGIR2017}. The model was implemented using deep neural networks and shown to outperform models that use pointwise scoring functions. This indicates that there are additional benefits to model document comparison at the feature level, in addition to the comparison at the loss level. 

%Hence we hypothesize that learning-to-rank models should compute the relevance score of a document to a query by comparison with other documents in the list at the feature level. Figure~\ref{fig:scoringloss} (b) presents an example that takes document pairs as input, and computes their relative preferences based on the joint features of the pairs in a past work~\cite{Dehghani:SIGIR2017}, which was shown to be more effective than pointwise scoring functions.

%Figure~\ref{fig:scoringloss} illustrates the notions of pointwise, pairwise, and groupwise scoring functions.
%\begin{itemize}
%\item Figure~\ref{fig:scoringloss}(a) describes pointwise methods, in which both scoring and loss functions are limited to a single document. Such methods include regression, classification and ordinal regression, and were generally found less effective for information retrieval applications~\cite{liu2009learning}.
%\item Figure~\ref{fig:scoringloss}(b) describes preference modeling methods, where scoring functions are trained based on pairwise document preferences~\cite{Cohen+al:1999, Dehghani:SIGIR2017} and which were shown to give better ranking accuracy than models using pointwise scoring functions.
%\item Figure~\ref{fig:scoringloss}(c) captures a large family of existing models with pointwise scoring functions and listwise loss (e.g., ListNet \cite{cao2007learning}, ListMLE \cite{xia2008listwise}, LambdaMART \cite{burges2010ranknet}, and AdaRank \cite{Jun+Hang:2007}). 
%\item Figure~\ref{fig:scoringloss}(d) shows how these models can be extended to support groupwise scoring functions, where all the documents are considered in both scoring and loss functions, which is the path we take in this paper.
%\end{itemize}

% Propose GSF
In this paper, we explore a general setting of \emph{groupwise scoring functions} (GSF) to enhance the direct comparison at the feature level. A GSF is designed to take multiple documents as input and scores them together based on the joint set of features of these documents. 
%Such a setting is contrasted to other settings in Figure~\ref{fig:scoringloss} (d).
While it is easy to define a GSF, it is unclear how to learn such a function from training data efficiently. Furthermore, even though we can train a GSF, how to use it to score a new list of documents during inference remains a challenge. This challenge is acknowledged in~\cite{Dehghani:SIGIR2017} and their method has a quadratic time complexity since all possible document pairs are evaluated during inference.

To solve these challenges, we propose a novel deep neural network architecture in the learning-to-rank setting. We design a sampling method that allows us to train GSF efficiently using standard neural network techniques like back-propagation. Furthermore, our formulation allows us to obtain a scalar value per document during inference using a Monte Carlo method efficiently.  More interestingly, our formulation is generic and we show that several representative learning-to-rank models can be formulated as special cases in our GSF framework.

%The output of GSF is the \emph{relative relevance score} of a document with respect to the other documents in a group. The final score of each document is computed by aggregating all the relative relevance scores in a voting mechanism. Then a  loss function can be defined between the final scores and labels for the entire document list and used to learn the GSF. Our proposed GSF setting is general and subsume both pointwise and pairwise cases. In particular, we show that several representative learning-to-rank models can be formulated as special cases in our GSF formulation.

%% Combination w/ tree-based models
%We choose to implement GSF using deep neural networks (DNNs), which can directly make use of both raw textual document and query representations, as well as derived numerical ones (e.g., match scores like BM25 or quality scores like PageRank). Thus, GSF can be viewed as a synthesis between the traditional learning-to-rank methods~\cite{liu2009learning} that make use of pre-defined numerical features and the recent deep semantic matching methods (e.g., DeepRank~\cite{DeepRank:2017}, DRMM~\cite{Guo+al:2016}, MatchPyramid~\cite{MatchPyramid:2016}) that learn relevance directly from the raw textual document and query representations. In this paper, we empirically demonstrate the value of such synthesis in two complementary settings.
 
%As we demonstrate, this makes GSF highly effective when large amounts of data are available, e.g., when large amounts of click data are available for training. 
%As we demonstrate, this makes GSF highly effective when large amounts of click data are available for training. 
%However, even in the scenarios when the number of training examples is limited, and no raw textual representations are available (e.g., in publicly available learning-to-rank datasets~\cite{DBLP:journals/corr/QinL13}), GSF can still lead to significant gains, when combined with the state-of-the-art tree-based models, e.g., LambdaMART \cite{burges2010ranknet}.

% Personal search scenario and experiments
%While the theoretical contributions of this paper generalize to any ranking scenario, in this paper we empirically validate the value of groupwise scoring functions in two complementary settings. 

We evaluate our proposed models in the following two scenarios. First, we show that our GSF can be used in the unbiased learning-to-rank setting~\cite{Joachims:WSDM17} to learn from a large amount of biased click data. The specific application in our paper is email search~\cite{carmel2015rank, dumais2003stuff, QingyaoAi:WWW2017, grevet2014overload}. An important characteristic of email search is that each user can only access their own email corpus, and TREC-like relevance judgements are no longer available~\cite{Wang+al:2018}. Therefore, click logs are the primary source of training data and unbiased learning-to-rank becomes critical for such applications. Second, we study GSF in the standard learning-to-rank setting. In this setting, we evaluate GSF using the LETOR data set MSLR-WEB30K~\cite{DBLP:journals/corr/QinL13}, in which the relevance judgments are obtained from human ratings, and a pre-defined feature set is provided. We show that our GSF perform reasonably well by themselves and can improve the state-of-the-art tree-based models in a \emph{hybrid} setting where the output of GSF is used as a feature for tree-based models.

%The unbiased learning-to-rank algorithms can overcome the bias in click logs but they are mainly designed on top of pairwise losses~\cite{Wang+al:2016,Joachims:WSDM17,Wang+al:2018}. In this paper, we propose a novel unbiased listwise loss function for our proposed listwise input models. 

%In summary, the contributions of our work are:
%\begin{itemize}
%	\item We introduce a novel formulation of \emph{groupwise scoring functions} that model cross-document comparison directly in scoring functions and implement it using deep neural networks.
%	\item We demonstrate that our GSF models can be viewed as a generalization of several representative learning-to-ranking algorithms.
%	\item We show that our GSF formulation can be used in unbiased learning-to-rank from click logs. We also propose a \emph{hybrid} approach that combines GSF with a tree-based model such as LambdaMART, and evaluate the effectiveness of this approach on a public dataset.
%\end{itemize}

% Commented by xuanhui@
% The rest of the paper is organized as follows. We first discuss the related work in Section~\ref{sec:related} and formulate groupwise scoring functions in Section~\ref{sec:problem_formuation}.
% Then we describe the deep neural network and our proposed methods in Section~\ref{sec:method}.
% Section~\ref{sec:relationship_with_others} discusses the relationship between our methods and existing learning-to-rank algorithms.
% Section~\ref{sec:eval} and~\ref{sec:results} describes the experimental design and evaluation using both proprietary and public data sets. Finally, we conclude the paper and discuss future work in Section~\ref{sec:conclusion}.
% End{xuanhui@}



==> proposed_methods.tex <==
%!TEX root=paper.tex

%Show that previous models are special cases in the current model
\section{The GSF Models}\label{sec:proposed_method}

A straightforward approach to learn a groupwise scoring function $f$ is to concatenate all features of documents in $D$ together and build a feed-forward network with output with size $n$ as the relevance prediction of the whole list. Such an approach, however, has two drawbacks: (1) The learned model is sensitive to document order; (2) The comparison is among all documents and this can make it difficult to learn the useful local comparison patterns. To overcome these drawbacks, we propose to limit the comparison within small groups and make the model invariant to the document order. In this section, we describe our model architecture, training, and inference for our GSF models built with DNNs.

\subsection{Model Architecture}

\begin{figure}
	\centering
	\includegraphics[width=3.5in]{./figure/groupwise.pdf}
	\caption{An example of Groupwise Scoring Functions (GSF) using permutations of size 2 in $\mathcal{S}$ for a $D$ with 3 documents.}
	\label{fig:groupwise}
\end{figure}

Our DNN architecture is shown in Figure~\ref{fig:groupwise}. It has a few components as follows.
% There are three components in the groupwise scoring design: the input document list, the groupwise scoring function, and the training algorithm.

\subsubsection{Input}
%\subsubsection{Fixed List Size}
%In this section, we first introduce our proposed DNN model for $f$ with listwise input and how to infer the score of each document with it.
%Then we discuss our loss function $l$ for learning to rank with different types of relevance judgments.
The input of our GFS models consists of a document list $D$ with $n$ documents. In order to use existing DNN toolkits such as TensorFlow\footnote{https://www.tensorflow.org/}, which use mini-batches with stochastic gradient descent (SGD) during training, we make a simplifying assumption that each DNN training example has a fixed number of documents $n$ and $n = |D|$. Such an assumption trivially holds in the click data setting where the top-$n$ documents per query is used. For a more general case, where the list sizes vary per query, we can apply padding or sampling strategy. For example, we randomly sample $n$ documents per query (where $n$ is smaller than the list size) to form a training example. When $n=2$, such a sampling strategy is similar to standard pairwise approaches where document pairs of a query are formed as training examples.
%  As our experimental results demonstrate, this strategy, while simple, is effective given enough training examples.

%\subsubsection{Model Architecture}\label{sec:dnn_voting}
\subsubsection{Groupwise Scoring Functions}\label{sec:dnn_voting}
Given a group size $m \leq n$, let $\mathcal{S} = \{\pi_1,\pi_2, ..., \pi_{|\mathcal{S}|}\}$ be all the permutations of the subset documents with size $m$ from $D$. The groupwise function $g$ takes $\pi_k$ as input and produces the intermediate scores 
$$[r_k^1, ..., r_k^m] = g(q, \pi_k).$$

The function $g$ can be implemented in multiple ways. In this paper, we implement $g$ using the DNN model in Section~\ref{sec:simple_dnn} as the building block. Specifically, we concatenate the features of $q$ and $d \in \pi_k$ to form an input vector $\bm{x}_{\pi_k}$.
For example, $\bm{x}_{\pi_k}$ would be the concatenation of $\bm{x}_q^{\text{embed}}$, $\bm{x}_{d_1}^{\text{embed}}$, $\bm{x}_{d_2}^{\text{embed}}$, $\bm{x}_{d_1}^{\text{dense}}$ and $\bm{x}_{d_2}^{\text{dense}}$ for $\pi_k=[d_1, d_2]$.
After that, we treat $\bm{x}_{\pi_k}$ as $\bm{h}_0$ and use the DNN in Equation~(\ref{equ:dnn}) to produce a latent vector $\bm{h}_{\pi_k} = \bm{h}_3$ . The final outputs of the group comparison is
\begin{equation}
g(q,\pi_k) = \bm{w}_g^T\bm{h}_{\pi_k} + \bm{b}_{g}
\label{equ:group_comparison_func}
\end{equation}
where $\bm{w}_{g}$ and $\bm{b}_{g}$ are the weight matrix and the bias vector for $g$. Please note that all weight parameters in the function $g(q, \pi_k)$ (in Figure~\ref{fig:groupwise}) are shared across all the groups in $\mathcal{S}$. It not only reduces the number of parameters in our DNN models, but also makes the model invariant to the input document order: any permutation of $D$ as input gives the same score for the same document after the voting mechanism below. 

\subsubsection{Final Scores by Voting}
In our GSF models, a small group of documents are compared and scored based on their feature vectors to predict which documents are more relevant in the group. Then the intermediate relevance scores from the individual groups are accumulated to generate final scores. Specifically, the final ranking score $s_d$ for $d \in D$ is accumulated by voting as 
\begin{equation}
s_d = \sum_{k=1}^{|\mathcal{S}|}\sum_{j=1}^{m} \bm{1}_{\pi_k^j=d} \cdot r_k^j 
\label{equ:group_func}
\end{equation} 
where $r_k^j$ is the intermediate score for the $j$-th document in $\pi_k$ and $\bm{1}_{\pi_k^j=d}$ is an indicator function that denotes whether $d$ is the $j$-th document in $\pi_k$. An example is shown in Figure~\ref{fig:groupwise} where we have $n = 3$ and $m = 2$.

%Let $\bm{s}$ be a score vector where $s_i$ denotes the ranking score of $d_i \in D_Q$, then we have
%\begin{equation}
%\bm{s} = f(q, D_Q) = F(\{f(\bm{x}_{(q,\pi_k)}) | \pi_k \in \mathcal{S}_Q\})
%\label{equ:F}
%\end{equation} 
%%where the output of $f$ is a $n$ dimensional vector.
%where $\bm{x}_{(q,\pi_k)}$ is the feature vector constructed with features for $d \in \pi_k$ and $F$ is an aggregation function that summarizes the outputs of $f$.
%

%where $\bm{c}_Q$ is a vector of binary labels where $y_i$ denotes whether $d_i$ has been clicked in $Q$.
%
%To show and analyze the effectiveness of the listwise input framework, we propose two ranking models with listwise input, which are the Groupwise Relevance Model and the Listwise Comparison Model.

%$\mathcal{S}_Q = \{\pi_1,\pi_2, ..., \pi_m\}$ be a set of sublists for $D_Q$ which covers all $d \in D_Q$ and each $\pi_k \in \mathcal{S}_Q$ has same number of documents. 
%The ranking scores for $d \in D_Q$ under the new framework is computed as

%where $F$ is an aggregation function that summarizes the outputs of $f$ and predict scores for each $d \in D_Q$.
%Let $T_Q = \{t_1,t_2, ..., t_n\}$ be another set of sublists for $D_Q$. $T_Q$ also covers all $d \in D_Q$ and each $t_v \in T_Q$ also has same number of documents.

%Inspired by the studies of pairwise models~\cite{Dehghani:SIGIR2017}, an intuitive way to build a listwise input model is to formulate the problem of ranking as a set of document comparisons. 

\subsection{Loss Functions for Training}\label{sec:loss_function}
Our GSF DNN models output a score for each document in the list. Intuitively, we can define listwise loss functions between the scores and labels to train the GSF models~\cite{cao2007learning}. In this section, we focus on two simple loss functions for two types of labels, binary relevance and graded relevance, leaving the study of other loss functions to the future.

\subsubsection{Loss for Binary Relevance}
Learning-to-rank with binary labels refers to the cases where each document is labeled as relevant or non-relevant. It is common when user clicks are used as labels. In this setting, it is important to define a loss function that can be used for unbiased learning-to-rank~\cite{Joachims:WSDM17, Wang+al:2018}.
%In this section, we address the concerns of learning from biased click data in the unbiased learning-to-rank framework. We follow previous work in this area~\cite{Joachims:WSDM17, Wang+al:2018}, and implement the local loss function in Equation~\ref{equ:local_loss} by taking the click bias into consideration. Previous work in learning-to-rank usually starts from formulating an unbiased performance metric and then translates it to an unbiased loss function. Inspired by this work, in this paper, we directly propose an \emph{unbiased loss function}.

Let $y_i$ be the binary label of whether the $i$-th document $d_i$ in $D$ is relevant. In GSF, the scores $\bm{s}$ are represented by an $n$-dimensional vector. We adapt the softmax cross entropy used in multi-class classification tasks to define our loss function as:
\begin{equation}
l(\psi,f) = - \sum_{i=1}^{n} y_i \cdot \log p_i
\label{equ:softmax_loss}
\end{equation}
where $p_i$ is the softmax of score $s_i$:
\begin{equation}
p_i = \frac{e^{s_i}}{\sum_{j=1}^{n} e^{s_j}}
\label{equ:softmax}
\end{equation}
The softmax loss is a listwise loss due to the dependency on other documents in the denominator in Equation~(\ref{equ:softmax}). An important property is that this function can be refined for unbiased learning-to-rank with click data. Specifically, we use the Inverse Propensity Weighting proposed in unbiased learning-to-rank to overcome click bias~\cite{Joachims:WSDM17, Wang+al:2018}. The IPW method estimates a weight $w_i$ \emph{for and only for} each \emph{clicked} document. The IPW version of softmax loss in Equation~(\ref{equ:softmax_loss}) is
\begin{equation}
l(\psi,f) = - \sum_{i=1}^{n} w_i \cdot y_i \cdot \log p_i = - \sum_{i: y_i = 1} w_i \cdot \log p_i
\label{equ:ipw_softmax_loss}
\end{equation}
The loss is well-defined because the sum is over only clicked documents, i.e., $y_i = 1$. As shown in the next section, this is not the case for the listwise loss used in ListNet~\cite{cao2007learning}.

% An alternative way to define the loss is using sigmoid cross entropy:
%\begin{equation}
%l(\psi,f) = - \sum_{i=1}^{n} y_i \cdot \log p_i + (1-y_i) \cdot \log(1-p_i)
%\label{equ:sigmoid_loss}
%\end{equation}
%where $p_i$ is the estimated click probability of $s_i$ computed with
%\begin{equation}
%p_i = \frac{1}{1 +  e^{-s_i}}
%\label{sigmoid}
%\end{equation}
%Note that the sigmoid cross-entropy is identical to the loss in Equation~\ref{equ:pointwise_loss}. It is thus a pointwise loss, since there is no dependency on other scores in the same input document list. 

\subsubsection{Loss for Graded Relevance}
In contrast to binary relevance, graded relevance is a multi-level relevance judgment and is commonly used in human-rated data sets. The loss for graded relevance is generally defined over document pairs.
%This paradigm is often used in the construction of public learning-to-rank datasets (e.g. MSLR~\cite{DBLP:journals/corr/QinL13}) where human experts were recruited to annotate the relevance of each query-document pair. 
%Entropy-based loss functions are not applicable in this case because the value of judgment labels only indicates document preferences but not document relevance.
We extend the commonly used pairwise logistic loss for a list as 
\begin{equation}
l(\psi,f) = \sum_{i=1}^{n}\sum_{j=1}^{n} \bm{1}_{y_i > y_j} \cdot \log (1 + e^{-(s_i - s_j)})
\label{equ:logistic_loss}
\end{equation}
where $y_i > y_j$ means the $i$-th document is more relevant than $j$-th document and the loss of a list is the sum of the loss of all pairs in the list. Please note that when $m=1$, GSF is actually a pointwise scoring function. In this case, the loss in Equation~(\ref{equ:logistic_loss}) boils down to a pairwise loss function. However, it becomes a listwise loss for the general GSF models when $m \geq 2$.



%where $y_i$ is the multi-level relevance label for $d_i$ and $p_{ij}$ is the probability that $d_i$ is more relevant than $d_j$ estimated by $s_i$ and $s_j$:
%\begin{equation}
%p_{ij} = \frac{1}{1 +  e^{s_j-s_i}}
%\label{logistic}
%\end{equation}
%The moitivation of our logistic loss function is to optimize $\bm{s}$ through maximizing the log likelihood of observed document preferences.

%Unbiased learing-to-rank was studied in \cite{Wang+al:2016, Joachims:WSDM17, Wang+al:2018} and the authors used a common method called Inverse Propensity Weighting (IPW). In this method, the propensity is the probability that a document relevance is \emph{observed} in the data. This is important for click data because a relevant document is not necessary clicked, meaning its relevance is not observed, and thus knowing the propensity is the base for unbiased learning. Formally, let $o_i \in \{0, 1\}$ denote whether the relevance of $d_i \in D$ is observed or not. In click data, $y_i = 1$ means $o_i = 1$, but $o_i$ is completely uncertain when $y_i = 0$. The unbiased loss functions for softmax cross entropy and sigmoid cross entropy are respectively
%\begin{equation}
%l(\psi,f) = - \sum_{i=1}^{n} \frac{\bm{1}_{o_i = 1}}{P(o_i = 1)} y_i \cdot \log p_i
%\label{unbiased_softmax_loss}
%\end{equation}
%and
%\begin{equation}
%l(\psi,f) = - \sum_{i=1}^{n} \frac{\bm{1}_{o_i = 1}}{P(o_i = 1)} \big[y_i \cdot \log p_i + (1-y_i) \cdot \log(1-p_i)\big]
%\label{unbiased_sigmoid_loss}
%\end{equation}
%Both loss functions are unbiased. However, the softmax loss in Equation~\ref{unbiased_softmax_loss} is defined over the set of documents where $y_i = 1$, while the sigmoid loss function in Equation~\ref{unbiased_sigmoid_loss} is defined over all documents with both $y_i = 1$ and $y_i = 0$. Given that it is uncertain about $o_i$ when $y_i = 0$, the sigmoid loss is not well-defined over the click data. In contrast, the softmax loss is well-defined since a document with $y_i = 0$ has a $0$ contribution to the loss.

%In this paper, similar to previous work, the propensity is estimated through a position bias model using result randomization~\cite{Wang+al:2018}. The unbiased softmax loss function in Equation~\ref{unbiased_softmax_loss} is used in our GRM and LCM models during training. %The IPW weights influence the weights in DNN through back-propagation.

% Unbiased learning 
%In personal search, a click behavior happens only when the user has read the result and believe it to be relevant. 
%A non-click behavior, however, could happen either when the user thinks the result is not relevant or when the user hasn't observed it.
%Similar to many retrieval problems~\cite{Joachims:WSDM17, craswell2008experimental, dupret2008user}, top results are more likely to be read and clicked in personal search. Therefore, search sessions with clicks on top results are more likely to be collected in click data~\cite{Wang+al:2016}.


%To learn a robust learning-to-rank model with biased data, Wang et al.~\cite{Wang+al:2016} adapted the framework of inverse propensity weighting (IPW) and proposed an unbiased global loss function for learning to rank in personal search as
%\begin{equation}
%\mathcal{L}_{\mathcal{Q}}(f) = \frac{1}{|\mathcal{Q}|}\sum_{Q\in\mathcal{Q}} \frac{P(Q)}{\hat{P}(Q)}l(Q,f) = \frac{1}{|\mathcal{Q}|}\sum_{Q\in\mathcal{Q}} w_Q \cdot l(Q,f)
%\label{equ:IPW}
%\end{equation} 
%where $\mathcal{Q}$ denotes all $Q$ in the click data, $P(Q)$ is the probability of observing $Q$ in $\mathcal{Q}$ without click biases and $\hat{P}(Q)$ is the probability of observing $Q$ in $\mathcal{Q}$ with click biases. 
%$\hat{P}(Q)$ is also referred as the propensity score of $Q$. 
%Assuming that the generation of click bias purely depends on the result positions, Xuanhui et al.~\cite{Wang+al:2016} estimated $w_Q = \frac{P(Q)}{\hat{P}(Q)}$ by randomizing result lists and collecting clicks on the same documents on different positions.
%In their experiments, each search session has at most one click, so the propensity weights for $Q$ can be represented with $\{w_i | i \in [1, \beta]\}$ where $w_i$ denotes the weight for $Q$ with clicks on the $i$th position. 
%For the training of the listwise input model, we adapted their unbiased learning-to-rank framework and reused their weighting schema. 

%The IPW framework, however, is not enough for unbiased learning on click data.
%An important problem that cannot be solved by the IPW is the uncertainty behind click labels.
%Usually, a click happens after the user read and believed the result to be relevant, while a non-click behavior happens either when the user didn't observe the result or when the user read the result and found it not relevant.
%Therefore, the feedback information from non-click behaviors are noisy.
%The IPW with a local loss $l(Q,f)$ that considers non-click behaviors is still biased.

%In Equation~\ref{equ:softmax_loss}, the softmax loss for non-clicked documents are 0 when $y_i=0$. Thus the softmax loss is defined on clicked documents only, while the sigmoid loss in Equation~\ref{equ:sigmoid_loss} has a non-zero loss on the non-clicked documents, i.e., $y_i = 0$. An unbiased version of the softmax loss is well-defined on the click data and thus used in our paper:
%\begin{equation}
%\mathcal{L}_{\mathcal{Q}}(f) = - \frac{1}{|\mathcal{Q}|}\sum_{Q\in\mathcal{Q}}  \sum_{i=1}^{n}w_i y_i \log p_i
%	\label{equ:IPW_softmax}
%\end{equation}
%where $w_i$ is the IPW estimated from the position bias model and depends on the clicked position only. Such a loss is provenly unbiased and we omit the details due to space limit.


\subsection{Training Efficiency}
There are $n! / (n - m)!$ possible permutations of a group with size $m$ in a list with size $n$, so directly using all permutations in $\mathcal{S}$ is computationally prohibitive. For efficient training, we conduct the following group sampling to reduce $\mathcal{S}$. For each training instance with document list $D$, we randomly shuffle it before feeding into the network. We only take the subsequences (instead of subsets) of size $m$ from the shuffled input to form $\mathcal{S}$. In this way, we reduce the size $|\mathcal{S}|$ from $n! / (n - m)!$ to $n$ subsequences: each starting at the $i$-th position and ending at $(i + m)$-th position in a circular manner. Each $d \in D$ appears in exactly $m$ groups.
Because all documents have an equal probability to be compared to others and to be placed as the $j$-th document in each sublist $\pi_k$, asymptotically, the GSF trained with our sampling strategy approaches (with enough training examples) the GSF trained with all permutations $\mathcal{S}$. Thus the GSF trained with sampling is insensitive to document order as well.

\subsection{Inference}
GSFs score multiple documents together, making it challenging to do inference with a GSF model. For ranking, the desired output is a ranked list. This can be done in a straightforward manner for pointwise scoring functions, but becomes non-trivial for GSF. In this section, we tackle this challenge by proposing our inference methods for the following two scenarios: fixed list size and varying list size. 

\textbf{Inference with Fixed List Size.} Given a fixed list size $n'$ at inference time, the most straightforward solution to do inference with GSF is to train the DNN model with the same list size $n=n'$. 
Thus, the score $f(d)$ for a document $d$ can be directly computed as $f(d) = s_d$ with Equation~(\ref{equ:group_func}).
%When $n' > n$, we can average the outputs of GRM in each sublist to get the final score for $d$ as 
%\begin{equation}
%	f(d) = \frac{1}{|S'|}\sum_{\pi' \in S'}s_d(\pi')
%\end{equation}
%where $S'=\{\pi'\}$ is the set of all possible document set $\pi'$ with length $n$ in the test list and $s_d(\pi')$ is the GRM score of $d$ in $\pi'$.
%If $d\notin \pi'$, then $s_d(\pi')=0$.

\textbf{Inference with Varying List Size.} When it is impossible to make $n= n'$ or the list size at inference time cannot be determined beforehand, it is hard to use the DNN architecture in training directly. In this case, we extract the group comparison function $g$ from GSF and use it to do inference. For each document $d$ in the inference list $D$, we compute its score $f(d)$ by the expected marginal score as
\begin{equation}
f(d) = \mathbb{E}_{\pi \in \mathcal{S}, \pi^i = d}~g(q,\pi) |_i
\label{equ:arbitrary_inference}
\end{equation}
where the expectation is over all possible permutations of size $m$ in $\mathcal{S}$ that contains document $d$ and $g(q,\pi) |_i$ is the $i$-th value of the function output. For example, when $m=2$, $f(d)$ can be rewritten as
\begin{equation*}
f(d) = \frac{1}{2|D|}\sum_{d' \in D}\big[g(q,d,d')|_1 + g(q,d',d)|_2\big]
\end{equation*}

The expectation in Equation~(\ref{equ:arbitrary_inference}) can be approximated effectively by sampling. For example, when $m=2$, we can randomly sample a couple of documents and use the average over the sampled documents. The larger the sample size is, the better this approximation becomes. In our experiments, we found that sample size $m$ for group size $m$ is good enough. Thus the inference can be done efficiently.

In fact, the case for fixed list size is a special case of the varying list size. When $\mathcal{S}$ contains all adjacent documents as groups, it is equivalent to sampling $m$ groups for each document and the document's position varies from 1 to $m$ in these $m$ groups. The score of the document is proportional to the sum of the corresponding values in these $m$ groups.

%In fact, $s_d$ in GRM is the sum of group 


\iffalse
\subsection{Listwise Comparison Model}\label{sec:dnn_dnn}

Although the GSF explicitly models the relativity at the input level with group comparisons, it is still limited.
When $\pi_k$ is smaller than $D$, each group comparison can only observe partial information of the whole list.
The voting step in Equation~(\ref{equ:group_func}) essentially assumes that the intermediate relevance scores from each comparison should have equal weights in the final results.
This, however, is a strong assumption. % when each attention score is computed only with a sublist of all the candidate documents.
Because we need to conduct group sampling for efficient model training and evaluation, it is inevitable that each document would be compared with documents from different subsets of the same list.
A fair document would receive a high relative score when compared to bad ones, while a good document could receive a relatively low score when compared to excellent ones.
Therefore, the relative scores from each group could be incomparable, which would consequentially make the voting process problematic.
Given this observation, we further propose a Listwise Comparison Model (LCM) to address these problems.

\begin{figure}
	\centering
	\includegraphics[width=3.5in]{./figure/listwise.pdf}
	\caption{An example of the Listwise Comparison Model (LCM) using permutations of size 2 in $\mathcal{S}$ for a $D$ with 3 documents.}
	\label{fig:listwise}
\end{figure}

The idea of LCM is to do document comparisons at the list level. Similar to GRM, LCM also conducts group comparisons.
Before the generation of the final ranking scores, LCM uses another layer of fully-connected network, which we refer to as the listwise comparison layer, to automatically compare the information obtained from each group and set weights to compute the final scores.
Formally, let $\bm{h}_{\pi_k}$ be the latent representation of each sublist computed from the groupwise model. 
We concatenate $\{\bm{h}_{\pi_k} | \pi_k \in \mathcal{S}\}$ to form a new vector $\bm{x}_{\mathcal{S}}$ and compute the final ranking scores as
\begin{equation}
\bm{s} = \bm{w}_{o}^T\bm{x}_{\mathcal{S}} + \bm{b}_{o}
\label{equ:listwise_func}
\end{equation}
% where $\bm{w}_{f}$ and $\bm{b}_{f}$ are a weight matrix and a bias vector.
%Now the score of $d_i$ is computed based on the information from the whole candidate set $D_Q$.
Figure~\ref{fig:listwise} illustrates this Listwise Comparison model (LCM) for $m=2$ and $n=3$.

LCM is a more faithful representation of the listwise input than GRM, since the score of each document in LCM is predicted based on the information from the entire list -- either explicitly in the group comparison layer or implicitly in the listwise comparison layer.
%Given any valid $\mathcal{S}$, all $d\in D$ will be compared with all $d \in D$ either explicitly in the group comparison layer or implicitly in the listwise comparison layer.
The listwise comparison layer gives the model the flexibility to learn weights for different sublists directly from training data. In fact, GRM is a special case of the LCM where the $i$-th column of the weight matrix $\bm{w}_o^{(i)}$ is the concatenation of
$$\{\sum_{j=1}^{|\pi_k|} \bm{1}_{\pi_k^j=d_i} \bm{w}_{g}^{(j)} | \pi_k \in \mathcal{S}\} $$
%$$\{\sum_{j=1}^{|\pi_k|} \bm{1}_{\pi_k^j=d_i} \bm{w_{g}^j} | \pi_k \in \mathcal{S}_Q \}$$
and $i$-th column of the bias vector $b_{o}^{(i)}$ is 
$$\sum_{k=1}^{|\mathcal{S}|}\sum_{j=1}^{|\pi_k|} \bm{1}_{\pi_k^j=d_i} b_{g}^{(j)}$$
%$$\sum_{k=1}^{m}\sum_{j=1}^{|\pi_k|} \bm{1}_{\pi_k^j=d_i} b_{g}^j$$
where a superscript $(j)$ means the $j$-th column in the matrices or vectors.

To train an LCM model, we also randomly shuffle the input document lists, as described in the previous section. Thus, asymptotically, LCM is also insensitive to document order.
\fi

